xCoT: Cross-lingual Instruction Tuning for Cross-lingual Chain-of-Thought Reasoning

Chain-of-thought (CoT) has emerged as a powerful technique to elicit reasoning in large language models and improve a variety of downstream tasks. CoT mainly demonstrates excellent performance in English, but its usage in low-resource languages is constrained due to poor language generalization. To bridge the gap among different languages, we propose a cross-lingual instruction fine-tuning framework (xCOT) to transfer knowledge from high-resource languages to low-resource languages. Specifically, the multilingual instruction training data (xCOT-INSTRUCT) is created to encourage the semantic alignment of multiple languages. We introduce cross-lingual in-context few-shot learning (xICL)) to accelerate multilingual agreement in instruction tuning, where some fragments of source languages in examples are randomly substituted by their counterpart translations of target languages. During multilingual instruction tuning, we adopt the randomly online CoT strategy to enhance the multilingual reasoning ability of the large language model by first translating the query to another language and then answering in English. To further facilitate the language transfer, we leverage the high-resource CoT to supervise the training of low-resource languages with cross-lingual distillation. Experimental results on previous benchmarks demonstrate the superior performance of xCoT in reducing the gap among different languages, highlighting its potential to reduce the cross-lingual gap.

==> mgsm.tex <==

\usepackage{arydshln} % or booktabs if you prefer
\begin{table*}[t]
    \centering
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{lrrrrrrrrrrrr}
    \toprule
    \textbf{Method} & En & De & Fr & Es & Ru & Zh & Ja & Th & Te & Bn & Sw & Avg. \\
    \midrule 
    GPT-3.5 (text-davinci-002)  \\
    \arrayrulecolor{lightgray}\tabucline[0.4pt on 3pt off 3pt]{-}
    Direct &  16.0 & 14.8 & 16.8 & 17.2 & 12.4 & 18.0 & 11.2 & 8.8 & 0.8 & 4.4 & 8.8 \\
    Native-CoT &  53.6 & 36.0 & 37.6 & 40.4 & 28.4 & 40.0 & 26.0 & 10.8 & 0.4 & 6.4 & 11.2\\ 
    En-CoT & 53.6 & 44.0 & 46.0 & 44.8 & 28.4 & 40.8 & 32.4 & 19.6 & 5.6 & 9.6 & 20.8\\
    Translate-En & 53.6 & 46.4 & 46.4 & 51.6 & 48.8 & 47.2 & 44.8 & 41.2 & 42.8 & 41.2 & 37.6 \\
    \arrayrulecolor{black}\midrule
    Bloom-7B   \\
    \arrayrulecolor{lightgray}\tabucline[0.4pt on 3pt off 3pt]{-} \addlinespace[0.1cm] 
    Direct & 22.0 & 18.8 & 19.6 & 20.0 & 22.0 & 19.2 & 16.0 & 16.8 & 17.6 & 17.2 & 15.6 \\
    Native-CoT & \bf 62.4 & 49.2 & 46.4 & 56.8 & 48.4 & 46.8 & 40.0 & 52.8 & 45.6 & 46.0 & 35.2 \\
    En-CoT & \bf 62.4 & 53.6 & 51.2 & 58.0 & 55.6 & 46.0 & 49.6 & 49.6 & 46.8 & 46.4 & 44.4 \\
    Translate-En &  \bf 62.4 & \bf 57.2 & \bf 55.2 & \bf 60.0 & \bf 59.6 & \bf 55.6 & \bf 50.0 & \bf 50.8 & \bf 49.6 & \bf 53.2 & \bf 51.2 \\
    \ourmethod{} &  \bf 62.4 & \bf 57.2 & \bf 55.2 & \bf 60.0 & \bf 59.6 & \bf 55.6 & \bf 50.0 & \bf 50.8 & \bf 49.6 & \bf 53.2 & \bf 51.2 \\
    \arrayrulecolor{black}  \midrule
Llama-2-7B   \\ 
    \arrayrulecolor{lightgray}\hdashline \addlinespace[0.1cm]
    Direct & 22.0 & 18.8 & 19.6 & 20.0 & 22.0 & 19.2 & 16.0 & 16.8 & 17.6 & 17.2 & 15.6 \\
    Native-CoT & \bf 62.4 & 49.2 & 46.4 & 56.8 & 48.4 & 46.8 & 40.0 & 52.8 & 45.6 & 46.0 & 35.2 \\
    En-CoT & \bf 62.4 & 53.6 & 51.2 & 58.0 & 55.6 & 46.0 & 49.6 & 49.6 & 46.8 & 46.4 & 44.4 \\
    Translate-En &  \bf 62.4 & \bf 57.2 & \bf 55.2 & \bf 60.0 & \bf 59.6 & \bf 55.6 & \bf 50.0 & \bf 50.8 & \bf 49.6 & \bf 53.2 & \bf 51.2 \\ 
    \ourmethod{} &  \bf 62.4 & \bf 57.2 & \bf 55.2 & \bf 60.0 & \bf 59.6 & \bf 55.6 & \bf 50.0 & \bf 50.8 & \bf 49.6 & \bf 53.2 & \bf 51.2 \\ 
    \arrayrulecolor{lightgray}\midrule
    Llama-2-13B   \\ 
    \arrayrulecolor{lightgray}\hdashline \addlinespace[0.1cm]
    Direct & 22.0 & 18.8 & 19.6 & 20.0 & 22.0 & 19.2 & 16.0 & 16.8 & 17.6 & 17.2 & 15.6 \\
    Native-CoT & \bf 62.4 & 49.2 & 46.4 & 56.8 & 48.4 & 46.8 & 40.0 & 52.8 & 45.6 & 46.0 & 35.2 \\
    En-CoT & \bf 62.4 & 53.6 & 51.2 & 58.0 & 55.6 & 46.0 & 49.6 & 49.6 & 46.8 & 46.4 & 44.4 \\
    Translate-En &  \bf 62.4 & \bf 57.2 & \bf 55.2 & \bf 60.0 & \bf 59.6 & \bf 55.6 & \bf 50.0 & \bf 50.8 & \bf 49.6 & \bf 53.2 & \bf 51.2 \\ 
    \ourmethod{} &  \bf 62.4 & \bf 57.2 & \bf 55.2 & \bf 60.0 & \bf 59.6 & \bf 55.6 & \bf 50.0 & \bf 50.8 & \bf 49.6 & \bf 53.2 & \bf 51.2 \\
    \arrayrulecolor{black} \bottomrule
    \end{tabular}}
    \caption{Multilingual evaluation results on the MGSM benchmark.}
    \label{tab:main_table}
\end{table*}

